Related Tasks can Share! A Multi-task Framework for Affective language

Expressing the polarity of sentiment as 'positive' and 'negative' usually have limited scope compared with the intensity/degree of polarity. These two tasks (i.e. sentiment classification and sentiment intensity prediction) are closely related and may offer assistance to each other during the learning process. In this paper, we propose to leverage the relatedness of multiple tasks in a multi-task learning framework. Our multi-task model is based on convolutional-Gated Recurrent Unit (GRU) framework, which is further assisted by a diverse hand-crafted feature set. Evaluation and analysis suggest that joint-learning of the related tasks in a multi-task framework can outperform each of the individual tasks in the single-task frameworks.

==> ablation.tex <==
\begin{table}[!ht]
    \caption{Pearson correlation coefficient for single-task learning (STL) and multi-task learning (MTL) frameworks for both sentiment classification and intensity prediction. }
    \centering
    \resizebox{0.48\textwidth}{!}
    {
    \begin{tabular}{c|c|c|c||c|c}
    % \cline{2-5}
        \multirow{2}{*}{Input} & & \multicolumn{2}{c||}{Sentiment Classification} & \multicolumn{2}{c}{Intensity Prediction} \\ \cline{3-6}
        & & DL (Softmax) & ML (SVM) & DL (Sigmoid) & ML (SVR) \\ \hline \hline
        \multirow{2}{*}{WE} & STL & \bf 0.384 & \bf 0.738 & \bf 0.804 & \bf 0.809 \\
        & MTL &  0.329 & 0.719 & 0.705 & 0.803 \\  \hline
        \multirow{2}{*}{Feat} & STL & \bf 0.379 & \bf 0.761 & \bf 0.813 & \bf 0.816 \\
        & MTL &  0.294 & 0.748 & 0.780 & 0.816 \\  \hline
        \multirow{2}{*}{WE + Feat} & STL & 0.361 & 0.745 & 0.821 & 0.818 \\
        & MTL & \bf 0.406 & \bf 0.772 & \bf 0.825 & \bf 0.830 \\  
    \end{tabular}
    }
    \label{tab:my_label}
\end{table}


% \begin{table}[!ht]
%     \caption{Pearson correlation coefficient for single-task learning (STL) and multi-task learning (MTL) frameworks for both sentiment classification and intensity prediction without using handcrafted features. }
%     \centering
%     \begin{tabular}{c|c|c||c|c}
%     % \cline{2-5}
%         & \multicolumn{2}{c||}{Sentiment Classification} & \multicolumn{2}{c}{Intensity Prediction} \\ \cline{2-5}
%             & DL (Softmax) & ML (SVM) & DL (Sigmoid) & ML (SVR) \\ \hline \hline
%         STL & \bf 0.384 & \bf 0.738 & \bf 0.804 & \bf 0.809 \\ \hline
%         MTL &  0.329 & 0.719 & 0.705 & 0.803 \\  
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}

% \begin{table}[!ht]
%     \caption{Pearson correlation coefficient for single-task learning (STL) and multi-task learning (MTL) frameworks for both sentiment classification and intensity prediction using only handcrafted features. }
%     \centering
%     \begin{tabular}{c|c|c||c|c}
%     % \cline{2-5}
%         & \multicolumn{2}{c||}{Sentiment Classification} & \multicolumn{2}{c}{Intensity Prediction} \\ \cline{2-5}
%             & DL (Softmax) & ML (SVM) & DL (Sigmoid) & ML (SVR) \\ \hline \hline
%         STL & \bf 0.379 & \bf 0.761 & \bf 0.813 & \bf 0.816 \\ \hline
%         MTL &  0.294 & 0.748 & 0.780 & 0.816 \\  
%     \end{tabular}
%     \label{tab:my_label}
% \end{table}

\begin{table}[!ht]
\caption{Comparison of actual seernet result and its replication }
\begin{tabular}{ccc}
 & Sentiment Classification & Intensity Prediction \\ \cline{2-3} 
\multicolumn{1}{c|}{Seernet Predictions} & \multicolumn{1}{c|}{\bf83.6} & \multicolumn{1}{c|}{\bf87.3} \\ \cline{2-3} 
\multicolumn{1}{c|}{Replication} & \multicolumn{1}{c|}{77.69} & \multicolumn{1}{c|}{82.99} \\ \cline{2-3} 
\end{tabular}
\end{table}
